A Markov Chain Model for the Decoding Probability of Sparse Network Coding

Random Linear Network Coding (RLNC) has been proved to offer an efficient communication scheme, leveraging an interesting robustness against packet losses. However, it suffers from a high computational complexity and some novel approaches, which follow the same idea, have been recently proposed. One of such solutions is Tunable Sparse Network Coding (TSNC), where only few packets are combined in each transmissions. The amount of data packets to be combined in each transmissions can be set from a density parameter/distribution, which could be eventually adapted. In this work we present an analytical model that captures the performance of SNC on an accurate way. We exploit an absorbing Markov process where the states are defined by the number of useful packets received by the decoder, i.e the decoding matrix rank, and the number of non-zero columns at such matrix. The model is validated by means of a thorough simulation campaign, and the difference between model and simulation is negligible. A mean square error less than $4 \cdot 10^{-4}$ in the worst cases. We also include in the comparison some of more general bounds that have been recently used, showing that their accuracy is rather poor. The proposed model would enable a more precise assessment of the behavior of sparse network coding techniques. The last results show that the proposed analytical model can be exploited by the TSNC techniques in order to select by the encoder the best density as the transmission evolves.

==> Annex.tex <==
\section{Annex}
\label{annex}

In this annex, we use simple combinatorial mathematics to derive the transition probabilities of the absorbing Markov chain that was previously discussed.

For any $(r,c)$ state, if the new packet includes any novel coefficient, the rank is always increased. The number of combinations that would change the state from $(r,c)$ to $(r+1,c+i), \quad i>0$ are:

\begin{equation}
N_{(r,c)}(r+1,c+i) = \mathbb{C}_{w-i}^c \; \mathbb{C}_{i}^{k-c} =  \binom{c}{w-i} \cdot \binom{k-c}{i}
\end{equation}

\noindent where $\mathbb{C}_{t}^n$ is the combination of $n$ elements taken $t$ at a time without repetition. 

In addition, the overall number of possible vectors are $\mathbb{C}_{w}^k$. Hence, the corresponding probability is:

\begin{multline}
p_{r,c}(1,j>0) = \frac{\binom{c}{w-i} \cdot \binom{k-c}{i}}{\binom{k}{w}} = \\ = \frac{\frac{c!}{\left(c-w+i\right)!\left(w-i\right)!} \cdot \frac{k-c!}{\left(k-c-i\right)!i!}}{\frac{k!}{\left(k-w\right)!w!}} = \\%\\= \frac{w!}{\left(w-i\right)! i!} \cdot \frac{c!}{\left(c-w+i\right)!} \cdot \frac{\left(k-w\right)!}{\left(k-c-i\right)!} \cdot \frac{\left(k-c\right)!}{k!} = \\ = \binom{w}{i} \cdot \prod_{t=0}^{w-i-1} \left(c-t \right) \cdot \frac{\prod_{t=w}^{c+i-1} \left(k-t \right)}{\prod_{t=0}^{c-1} \left(k-t \right)} =\\
= \binom{w}{i} \cdot  \frac{\prod\limits_{t=0}^{w-i-1} \left(c-t \right) \cdot \prod\limits_{t=c}^{c+i-1} \left(k-t \right)}{\prod\limits_{t=0}^{w-1} \left(k-t \right)}
\end{multline}

On the other hand, if the new packet does not include any new coefficient, the corresponding vector could be either linearly dependent or independent, and this is established by $\vartheta$. The combinations that do not increase the number of already received coefficients is $\mathbb{C}_{w}^c$. Hence, the probability of staying at the current state, $(r,c)$ is:

\begin{multline}
p_{r,c}(0,0) = \vartheta_q(r,c,w) \frac{\binom{c}{w}}{\binom{k}{w}} = \vartheta_q(r,c,w) \frac{\frac{c!}{\left(c-w\right)! w!}}{\frac{k!}{\left(k-w\right)! w!}} = \\ = \vartheta_q(r,c,w) \prod\limits_{t=0}^{w-1} \frac{c-t}{k-t}
\end{multline}

While the probability of going to $(r+1,c)$ can be calculated as follows:

\begin{multline}
p_{r,c}(1,0) = \left[ 1- \vartheta_q(r,c,w)\right] \frac{\binom{c}{w}}{\binom{k}{w}} = \ldots = \\ = \left[1-\vartheta_q(r,c,w) \right] \prod\limits_{t=0}^{w-1} \frac{c-t}{k-t}
\end{multline}

Whenever a packet is received the rank can only increase in one single unit, and thus, $p_{r,c}(i,j) = 0, \quad i > 1$. Likewise, the number of novel coefficients per packet cannot be larger than $w$, so $p_{r,c}(i,j) = 0, \quad j > w$.

